Helping Visually Impaired People Take Better Quality Pictures

Perception-based image analysis technologies can be used to help visually impaired people take better quality pictures by providing automated guidance, thereby empowering them to interact more confidently on social media. The photographs taken by visually impaired users often suffer from one or both of two kinds of quality issues: technical quality (distortions), and semantic quality, such as framing and aesthetic composition. Here we develop tools to help them minimize occurrences of common technical distortions, such as blur, poor exposure, and noise. We do not address the complementary problems of semantic quality, leaving that aspect for future work. The problem of assessing and providing actionable feedback on the technical quality of pictures captured by visually impaired users is hard enough, owing to the severe, commingled distortions that often occur. To advance progress on the problem of analyzing and measuring the technical quality of visually impaired user-generated content (VI-UGC), we built a very large and unique subjective image quality and distortion dataset. This new perceptual resource, which we call the LIVE-Meta VI-UGC Database, contains $40$K real-world distorted VI-UGC images and $40$K patches, on which we recorded $2.7$M human perceptual quality judgments and $2.7$M distortion labels. Using this psychometric resource we also created an automatic blind picture quality and distortion predictor that learns local-to-global spatial quality relationships, achieving state-of-the-art prediction performance on VI-UGC pictures, significantly outperforming existing picture quality models on this unique class of distorted picture data. We also created a prototype feedback system that helps to guide users to mitigate quality issues and take better quality pictures, by creating a multi-task learning framework.

==> main_files/background_dg.tex <==

\input{fig/dataset_collage}

\section{Related Work}\label{sec:background}
\noindent\textbf{Image Quality and Distortion Datasets:}
The most heavily-used datasets in image quality research remain older corpora of synthetically generated distortions of natural pictures. Since synthetic distortions are quite different from authentic, real-world distortions, NR-IQA models trained on them perform poorly on real content \cite{clive}. Such ``legacy" datasets include LIVE \cite{hamidLiveDB}, CSIQ \cite{csiqdata}, TID-2008 \cite{ponomarenko2009tid2008}, and TID-2013 \cite{tid2013}. These contain very few ($< 30$) unique picture contents that have been synthetically distorted using single kinds of quality impairments (JPEG, Gaussian blur, etc.). As such, they do not capture the complex kinds of distortions that generally arise in natural scenarios. 

Recent datasets such as Live Challenge \cite{clive}, KonIQ \cite{koniq}, and LIVE-FB \cite{paq2piq} have tried to address these problems by obtaining subjective labels on much larger numbers of UGC images affected by naturally-occurring distortions. While these resources contain subjective quality labels, they do not include labels on distortion types, except for the smaller LIVE Challenge dataset \cite{clive}, which contains both quality and distortion labels on about $1200$ images captured with mobile devices.  The Flickr-Distortion dataset \cite{flickrdist} contains synthetic distortion labels on $804$ Flickr UGC images, but it does not contain any quality labels, and it has not been made public. The VizWiz-QualityIssues \cite{vizwiz} dataset is the only available resource that contains images taken by visually challenged users, and that also contains distortion labels for some common types of quality impairments and aesthetic flaws. However, since it lacks picture quality scores and supplies only 5 subjective distortion scores per image, it cannot be used in its current form for our purposes. 
The lack of any substantial UGC dataset (captured by visually challenged users or otherwise) containing both quality scores as well as distortion labels further motivated us to conduct a large-scale psychometric study of the perceptual quality and distortions present in typical VC-UGC. The dataset we created is $33$ times larger than any picture quality and distortion labelled dataset, and it is the only dataset of this kind that targets the area of assisting the visually  challenged. 

\noindent\textbf{Image Quality Models:}
For this application, we are not interested in full-reference (FR) image quality models like SSIM \cite{ssim}, which require the presence of pristine reference images to predict relative picture fidelity. Instead, we require NR-IQA (blind) models, which have recently achieved significant successes. Popular NR-IQA models include BRISQUE \cite{brisque}, NIQE \cite{niqe}, CORNIA \cite{cornia}, and FRIQUEE \cite{friquee}, which use ``handcrafted" statistical features to train shallow learners, typically SVRs, to predict quality. These models work well on legacy single synthetic distortion datasets \cite{hamidLiveDB, tid2013, ponomarenko2009tid2008} but perform poorly on real-world, UGC data \cite{koniq, paq2piq}. Deep NR-IQA models \cite{ghadiyaram2014blind, deepConvIQA, bosseDeepIQA, fullyDeepIQA} have also been developed that perform quite well on synthetic distortion datasets, but they struggle on UGC datasets like LIVE-Challenge \cite{clive} and LIVE-FB \cite{paq2piq}. An advanced deep model called PaQ-2-PiQ \cite{paq2piq} leverages relationships between local and global quality to achieve current SOTA performance on the largest and most comprehensible datasets. A few multi-task models like IQA-CNN++ \cite{cnniqapp} and QualNet \cite{qualnet} are available, that use relationships between quality and distortion features in a network to predict both picture quality scores and distortion categories. Again, these multi-task models perform well on synthetic datasets, but struggle on real-world UGC pictures and distortions. The authors of \cite{vizwiz} used an Xception backbone trained on ImageNet \cite{imageNet} to predict distortions on the VizWiz pictures and achieved promising results.   

\noindent\textbf{Assisting the Visually Challenged:}
Over the last decade, several applications have been developed to help visually challenged users capture better images. Most of these applications were built for visual recognition tasks \cite{taptapsee, easysnap, OGvizwiz}. \textit{TapTapSee} \cite{taptapsee} helps a user take focus-adjusted images, whereas applications like \textit{VizWiz Ver2} \cite{OGvizwiz} and \textit{EasySnap} \cite{easysnap} use simple darkness and blur detection algorithms. These all provide audio feedback after capturing an image, targeting object recognition. The authors of \cite{assisted_framework} developed an assisted photography framework to help users better frame their photos, using an image composition model to assess aesthetic quality. The \textit{Scan Search} \cite{scansearch} application uses the Lucas-Kanade \cite{lucaskanade} optical flow method to track feature points and determine the stability of the camera. The most stable frames are sent for online object detection. Both provide automatic selection of a best image. The authors of \cite{vizwiz} also developed algorithms to detect the recognizability and answerability of images captured by blind users, for image captioning and visual question answering applications. None of this is predicated on perceptual models or trained on human data. The absence of any robust model that can predict distortions that commonly afflict VC-UGC, and that can provide feedback on perceptual quality, motivated us to create one of our own.


==> main_files/dataset_3.1_acb.tex <==
% \input{dataset_collage.tex}
% \vspace{-0.5em}
\section{Dataset and Human Study}\label{sec:dataset_humanstudy}
% \vspace{-1em}
This section elaborates the construction of our new VC-UGC dataset and details the online human study by which we collected subjective quality labels. The proposed dataset contains $39,660$ images and $39,660$ patches extracted from them, half of which are salient patches, the other half cropped at random. We also collected $2.7$M qualilty ratings and distortion labels on them. This dataset, comprising VizWiz images, is larger than previous synthetic legacy datasets \cite{hamidLiveDB, tid2013, ponomarenko2009tid2008}, and significantly larger than any UGC dataset containing both quality and distortion labels \cite{clive}. It is also the first quality-focused dataset dedicated towards developing assistive technology for visually challenged photographers.    

\subsection{Constructing the Dataset}\label{dataset}
\subsubsection{Building upon VizWiz}
VizWiz \cite{Gurari2018VizWizGC} was the first publicly available dataset containing content generated by blind users. The images in the dataset (Fig. \ref{fig:exemplarFLIVE}) were generated under real use conditions via the VizWiz mobile application \cite{OGvizwiz}. As the main purpose of the application was to submit images for image captioning and to answer visual questions, it addresses a practical need for visually challenged users, and is a suitable platform on which to develop quality-perceptive assistive technology. The authors of \cite{vizwiz} used the same dataset to collect some common quality (blur, exposure) and aesthetic labels (framing, obstruction, orientation) along with information on image recognizability. To the best of our knowledge, this was the first attempt to develop a dataset of this kind. A deeper analysis of the data collected revealed important insights on VC-UGC images. The authors considered blur and framing to be the most prevalent flaws of VC-UGC content that render images unrecognizable. They also carried out a detailed analysis on the correlations between the different impairments, the relationships between recognizability and distortions, and pointed out crucial directions that research in this area should progress.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
However, that work did not address important aspects of the VC-UGC problem, which we seek to address by the development of a large new dataset and VC-UGC specific VQA algorithms we create on it. These models address technical distortions such as blur, over/under exposure, and noise, but not aesthetic flaws such as framing, mood, and content selection. While the latter are important, they involve different capture problems and perceptual processes and should be treated differently \cite{paq2piq}. 
% and hence should be studied individually \cite{paq2piq}, (b) natural quality distortions are diverse and just blur, bright, and dark are inadequate to cover the spectra, (c) five distortion ratings on each image is unreliable for consensus in an online crowdsourced study as has been pointed out in previous quality studies \cite{patchvq}, and (d) no global or local perceptual quality feedback was included in the dataset, and distortion and quality do not always correlate.  

\input{fig/data_stats}

\subsubsection{Categorizing Distortions}
As mentioned previously, natural distortions are extremely diverse and commingle with each other, making it hard to exhaustively categorize them \cite{clive, koniq}. Since the images in our dataset were captured by visually impaired persons, there is a prevalence of heavy distortions. Among these, we chose to focus on the most common and identifiable ones. This resulted in five major categories: focus blur (`blurry'), motion blur (`shaky'), overexposure (`bright'), underexposure (`dark'), and noise (`grainy'). We also included two other categories: `none' (signifying the absence of any distortion) and `other' (distortions that are non-identifiable or cannot be categorized as being one of the other options).

\subsubsection{Cropping Patches}
Relationships between local and global spatial quality have been shown to be important and, when modeled, lead to improved quality predictions \cite{paq2piq, patchvq}. Here, we carry these ideas further by studying the impact of the choice of patches on quality prediction. To do this, we divided the entire dataset into two random halves. On half the images, a random patch was cropped to $40\%$ of each its linear spatial dimensions. On the other half, the most visually salient patch of the same ($40\%$) dimensions was cropped. The SOTA pyramid feature attention network \cite{pyramidsal} was used to create saliency maps, from which the most salient patch was cropped. All of the patches have the same aspect ratios as the original image they were cropped from (Fig. \ref{fig:egPatches}).

\subsubsection{ORBIT Data}
To study the cross-dataset performance of our model and its applicability to video tasks, we also created a separate, smaller dataset containing images extracted from the ORBIT database \cite{orbit}. The ORBIT dataset includes videos captured by visually challenged users, with the identification of common objects as the subject, under two environmental conditions -  clean and cluttered. We selected $59$ types of objects at random, and from each we selected two videos (one clean and one cluttered). We then sampled each video at one frame per second, collecting a total of $2,235$ frame images in total (Fig. \ref{fig:exemplarFLIVE}). As before, we then collected global quality ratings on these to form the auxiliary ORBIT images dataset.   
\input{fig/crop_v_patches}




==> main_files/dataset_3.2_acb.tex <==
\subsection{Subjective Quality and Distortion Study}\label{sec:human_study}
Amazon Mechanical Turk (AMT) is a well-established crowdsourcing platform for subjective quality studies \cite{paq2piq, patchvq, vizwiz, clive, livevqc}. Our human study was carried out in three stages of data collection - image, patch, and ORBIT sessions. Overall, $3,945$ subjects participated in the study and, after rejection and cleaning, we collected an average of around $34$ ratings on each image and each patch. Our study was accessible to all platforms and geographical locations.

\subsubsection{AMT Study Design}
The workflow of the study is shown in Fig. \ref{fig:AMTdesign}. The subjects, who were assumed to have normal/corrected vision, were asked to participate in two tasks - rating image quality, and identifying the distortions present in the images. Each subject was asked to read two separate sets of instructions, one for each task, followed by a quiz to assess their understanding of the tasks at hand. After successfully passing the quiz, they experienced a training phase containing five exemplar distorted images, to help them become familiar with the task. The image was displayed on the left and the rating section on the right. The top half of the rating section displays a rating bar which allowed the subjects to tender overall quality scores on a continuous scale from $0-100$ using a sliding cursor. On the bottom half, they were provided seven options to choose the distortion(s) that they deemed present in the image, from among the options discussed earlier (Sec \ref{dataset}). During the testing phase, each subject rated $110$ images. After they completed the study, they were asked to complete a questionnaire regarding the study conditions and their demography. 
\input{fig/study_workflow}
\subsubsection{Subject Rejection}
As has been observed in previous studies, online crowdsourcing carries the risk of distracted, inadequately equipped, disengaged, or even frankly dishonest subjects, so there is often a high percentage of unreliable labels. Thus, we used various strategies to screen the subjects using criteria applied both during and after the study. 

\noindent \textbf{During Task:} During the instructional phase, we checked whether the subject's browser window, browser and OS version, and zoom (non-magnified) condition satisfied our requirements, as stated in the instructions. If they did not, their participation was ended. To detect dishonest workers, at the halfway point of each testing phase, we processed the scores already given to determine whether they had been giving consistent ratings, were only nudging the slider slightly, or were supplying random, haphazard scores. This was determined using both assigned quality scores and distortion labels. 

\noindent \textbf{Post Task:} Of the $110$ images viewed in a session, $5$ were repeated at different locations in the viewing sequence. A subject was rejected if their ``repeat" scores were not consistently similar to the scores given the first time. We also included $5$ images selected from the LIVE-FB dataset \cite{paq2piq} as ``golden" examples with reliable scores already available. We further screened the subjects by checking whether their ratings adequately matched the golden ones. 

Overall, we rejected the scores given by $814$ of the subjects. 

\subsubsection{Data Cleaning}
The remaining scores after subject rejection were subjected to a series of data cleaning steps: \textbf{(1)} We removed $43$ images ($1.3K$ ratings) that had a constant color and thus served no purpose for our study. \textbf{(2)} Ratings provided by subjects who did not wear their prescribed lenses during the task were also removed ($0.9\%$), since uncorrected vision might affect perceived quality. ``In-the-wild" datasets do not always impose this criterion. However, in this context, where we are trying to supply accurate feedback so that users can actively improve their photographs, this step is important. \textbf{(3)} We further applied the ITU-R BT.500-14 \cite{itu_standard} (Annex 1, Sec 2.3) subject rejection protocol to screen the outlier subjects, resulting in an additional $56$ subjects being rejected. \textbf{(3)} For each image and patch, we also rejected outliers from the individual score distributions, as follows. We first calculated the kurtosis \cite{kurtosis} to determine the normality of the scores. If they were determined to be normal, the Z-score outlier rejection method \cite{modzscore} was applied. Otherwise, the Tukey IQR method \cite{tukey1977exploratory} was applied. Overall, including all of the subject and score outlier rejections, around $1.7\%$ of the ratings were tossed. Following all of the data cleaning, we were left with about $2.7$M subject scores ($1.36$M on images, $1.33$M on patches) on VizWiz images, and an additional $76$K ratings on the ORBIT image dataset, which includes only whole images.   

\subsubsection{Data Analysis}\label{sec:data_analysis}
\noindent \textbf{Inter-subject quality consistency:} An inter-subject consistency test \cite{paq2piq, patchvq} was carried out by randomly dividing the entire subject pool into two disjoint sets of equal size, then calculating the Spearman Rank Correlation Coefficient (\textbf{SRCC}) \cite{kendall1948rank} between the two corresponding sets of MOS (mean opinion score). The average SRCC over $50$ such random splits yields a useful measure of inter-subject consistency. For our data, the average SRCC on VizWiz images was \textbf{0.93}, on patches was \textbf{0.90}, and on ORBIT images was \textbf{0.93}. Among the patches, the average SRCC on the random patch set was \textbf{0.87}, but for the salient patches was \textbf{0.92}, hence the ratings on salient patches were more consistent. The high consistency of quality scores across all the different sets substantially validates the efficacy of our data collection and subject rejection processes.

\noindent \textbf{Intra-subject quality consistency:} Each subject rated 5 ``golden" images. We computed the Linear Correlation Coefficient (LCC) \cite{pcc} between the mean of their ratings with the original scores. The median PCC value over all subjects was \textbf{0.90} for the VizWiz image study, \textbf{0.90} for the patch study, and \textbf{0.87} for the ORBIT study. Again, these high correlations help validate our overall subjective study protocol.

\noindent \textbf{Patch vs Image quality:} Fig. \ref{fig:patchCorrel} shows scatter plots of image MOS against patch MOS, including for the two different kinds of patches. The SRCC between image and patch MOS was \textbf{0.84} indicating a strong relationship between local and global image quality. The SRCC between image MOS and random and salient patch MOS was \textbf{0.82} and \textbf{0.86}, respectively, again indicating that salient patches could play a stronger role when representing global picture quality. This may be because some distortions are salient, and/or that distortions on salient regions are more annoying. 

\input{fig/vid_vs_vpatch}

\noindent \textbf{Distortion Score Analysis}
Unlike quality scores, the distortion labels are binary. To conduct a consistency analysis, we converted the binary labels into probabilistic values for each image by dividing the number of positive labels of each distortion by the total number of labels collected, hence each distortion category takes values between $0$ and $1$. We then computed the correlations between the resulting vectors. The average SRCC (inter-subject consistency) values for each of the respective distortion categories were: blurry (\textbf{0.75}), shaky (\textbf{0.62}), bright (\textbf{0.68}), dark (\textbf{0.60}), grainy (\textbf{0.35}), and none (\textbf{0.85}). It may be observed that some distortion categories were harder to consistently identify than others. The high agreement on `none' shows that it is easier to determine the absence of distortions. Similarly, the SRCC values computed between image and patch distortions were: blurry (\textbf{0.73}), shaky (\textbf{0.68}), bright (\textbf{0.60}), dark (\textbf{0.62}), grainy (\textbf{0.46}), and none (\textbf{0.73}). The lower correlations for some distortions (like `dark') suggests that the perception of distortions that are globally apparent may be more weakly impacted by local quality. 

\noindent \textbf{MOS and Distortion Distributions}
Fig. \ref{fig:MOShists} (top) plots the MOS distribution of the images in the VizWiz and ORBIT datasets. Fig. \ref{fig:MOShists} (bottom) shows the proportional distribution of distortion ratings in the two datasets. As expected, `blurry' seems to be the most prominent distortion in both datasets. Overall, ORBIT seems to contain more images of higher quality and with fewer distortions. Also, `grainy' and `dark' images, which occurred less often, are associated with less consistent ratings and are thus harder to predict. The non-uniform distribution of distortion types makes it harder to train a model which can perform equally well on all classes.    

\input{fig/mos_dist}



==> main_files/intro_acb.tex <==
\section{Introduction}
Computer vision breakthroughs have the power to build community and make technologies more accessible at the largest scales. One such example is making social media more accessible to visually challenged people. Being able to automatically understand picture and video content could benefit low-vision/blind users by AI-driven assistance when selecting pictures to upload on social media. Studies \cite{visstudy1, visstudy2, visstudy3, visstudy4} have shown that they often rely on friends for this task, making them feel vulnerable and/or disempowered. These studies have also shown that the visually impaired often ask for information about, and assistance with picture quality. Using automatic picture quality raters developed on large-scale perceptual databases to supply guidance and feedback could help them capture higher-quality pictures to upload on social media. 
Given the huge amount of user-generated picture and video content flooding online social and streaming media platforms~\cite{tiktok}, concerns about being able to assess and control the technical visual quality of this data have generally continued to increase. While a variety of successful recent No-Reference Image Quality Assessment (NR-IQA) models (those that do not require a reference to compare against) ~\cite{paq2piq, nima, cnnIqa} are available that can predict perceptual picture quality with reasonable accuracy, it remains an incompletely solved problem. 

\input{fig/fig_opening}

Given these kinds of visual quality tools, it seems apparent that they could be applied to assist visually challenged users for a variety of tasks, including object recognition, image captioning, visual question answering, and capturing high-quality photographs that the users can confidently share with others. While there has been progress on these topics \cite{vizwiz, OGvizwiz, scansearch, taptapsee}, the practical problem of helping low-vision/blind users capture high quality images remains unsolved. In our view, an appropriately designed NR-IQA predictor, that is capable of providing meaningful feedback, could help visually challenged users engage more frequently and confidently in the sharing of visual social media, and less reliant on manual assistance.

In photography, there is no ideal content against which to compare a picture being captured, NR-IQA models are the necessary tools that should be used to assess and give feedback as pictures are being captured, thereby helping visually challenged users generate satisfactory content. NR-IQA models can be designed to predict both the perceptual quality and distortion types, based on perceptually relevant `quality-aware' statistics of captured pictures \cite{brisque}. However, modeling the quality of natural images captured under natural conditions has proven to be a challenging problem \cite{paq2piq, nima, cnnIqa}. Moreover, pictures captured by visually challenged users, without any guiding feedback, usually suffer from high levels of distortion \cite{vizwiz}. Since state-of-the-art (SOTA) NR-IQA predictors have been designed and trained on datasets containing pictures captured by users generally having normal vision, they perform poorly at predicting the quality of visually challenged user-generated content (VC-UGC). 

As part of assisting visually impaired people to take better pictures, such a feedback system should also be able to describe the distortions that are occurring as pictures are being captured. Since distortions arise in many forms because of imperfect capture devices, focusing issues, stabilization problems, and the impact of sub-optimal lighting conditions, all amplified in this scenario, this problem is also quite different. Moreover, multiple distortions often intermix, making them harder to identify and classify. It is quite important to understand that the technical degree of distortion is not the same as perceptual quality, since the latter is also deeply affected by the content and by perceptual processes such as masking \cite{mseLoveLeave, vpooling}. Accomplishing both tasks for this application is both important and more difficult. It should be noted that pictures captured by visually challenged users also suffer from aesthetic flaws such as incorrect framing or orientation, which have been studied extensively leading to assistive applications like \cite{assistframework}, \cite{easysnap}, and \cite{OGvizwiz}. Here, our work focuses on helping users to improve the perceptual quality  of their captured and shared pictures, rather than photographic aesthetics, although ultimately, a feedback system should be able to assist visually impaired users to improve both of these aspects.

Another challenge of creating accurate IQA models is the need for large and appropriately labeled datasets.A variety of public image quality datasets are available, which has helped drive the development of NR-IQA predictors that can perform well on naturalistic pictures \cite{paq2piq, nima}. However, these do not contain pictures taken by visually challenged users, which are different in important ways, and these algorithms generally deliver poor prediction performance on VC-UGC \cite{vizwiz}. Several datasets are available that contain labels on picture distortion categories. For example,  VizWiz-QualityIssues \cite{vizwiz} has labels for six categories of quality and aesthetic flaws on images collected using the VizWiz app \cite{OGvizwiz}. The ORBIT \cite{orbit} dataset contains videos taken by visually challenged users, but their target is providing object recognition. We have been unable to find any VC-UGC dataset that has subjective image quality labels, hence we were motivated to build one to assist predictive modeling efforts.

Recent work on perceptual IQA \cite{paq2piq} and VQA \cite{patchvq} has shown that modeling the relationship between local and global distortions can lead to better visual quality predictions. Hence we built a Visually Challenged UGC dataset that is comprised of images taken from VizWiz, along with both randomly selected and salient patches extracted from these images. We also conducted a large-scale visual psychometric study on both the images and extracted patches, using Amazon Mechanical Turk (AMT), whereby we collected human subjective quality scores and distortion labels. This large dataset enabled us to design new IQA models that can accurately predict perceptual quality scores and also categorize distortions. We have used these learned models to build a feedback system to assist visually challenged users in taking better pictures. 

The contributions we make towards advancing progress on this highly impactful but challenging problem are summarized below: 

\begin{packed_enum}
\item \textbf{We built the largest subjective image quality and distortion database targeting  pictures captured by visually challenged users.} This new resource contains about $40$K images and $40$K patches (half randomly selected and half salient). We conducted a large-scale subjective picture quality study on them, where we collected $2.7$M quality labels and an equal number of distortion labels. This is also the largest publicly available distortion classification dataset. We also collected about $7$5K ratings on $2.2$K ORBIT images (frames extracted from ORBIT \cite{orbit} videos). (Sec.~\ref{sec:dataset_humanstudy})
\item \textbf{We created a state-of-the-art blind VC-UGC picture quality and distortion predictor.} Using a deep neural architecture based on the recent PaQ-2-PiQ model \cite{paq2piq}, we created a multi-task system that is able to predict both the perceptual quality of pictures captured by visually impaired users, as well as the presence and degree of five common picture distortions. Since the new model is trained on patches, we are also able to use it to predict spatial maps of both quality and of distortion types. The new model, which we refer to as P2P++, achieves top performance on the new dataset (LIVE-VizWiz) as well as on the LIVE-ORBIT mini-dataset when compared to SOTA NR-IQA models. (Secs.~\ref{sec:modeling} and \ref{sec:cross_data})
\item \textbf{Using the multi-task model, we also created a unique prototype feedback system to assist visually challenged users to take better quality pictures.} We use the outputs of the multi-task model to generate suitable feedback on overall quality, as well as prominent distortions, to guide visually impaired users, along with suggestions on how to mitigate quality issues. We also study how the obtained spatial distortion maps might be used to generate more sophisticated feedback. 
\end{packed_enum}




==> main_files/modeling_4.1.tex <==
\section{Modeling and Experiments}\label{sec:modeling}
Our goal is to create an application which can accurately predict and accordingly provide feedback on the perceptual quality and distortions present in a picture. Towards this end, we designed efficient model architectures able to predict quality and distortions, while accounting for local-to-global percepts. Our model is able to analyze quality and distortion types both separately and together in a  multi-task framework. 
\subsection{Data pre-processing}\label{sec:preprocess}
Unlike the quality scores, which could be used in their raw form, the distortion labels had to be transformed into suitable output labels for training. Since distortion type prediction is a classification task, binarizing the labels was our first choice. We considered multiple options to decide a threshold on the per-distortion proportions of ratings. The authors of \cite{vizwiz} considered $40\%$ ($2$ out of $5$) agreement to affirm the presence of a distortion. Since there were no perceptual principles to guide us, we experimented with three thresholds values: $0.3$, $0.4$, and $0.5$ and assumed the top three distortions (highest proportions of the total number of labels) to be present. An inter-subject consistency analysis on the binarized labels found that the SRCC values dropped by $17\%$--$34\%$ as compared to those obtained on the probabilistic values in Sec. \ref{sec:data_analysis}. Similarly, we noticed a drop of $27\%$--$44\%$ of correlation between assigned patch vs image distortion classes, as compared to the probabilistic approach. Among all the binarization strategies, the `max-three' approach led to the worst correlation values. Moreover, as the thresholds were increased, the distortion distributions became more skewed, leading to worse predictions. These results made sense in view of research on model robustness, which has shown that, for classification tasks, hard labels tend to lead to higher confidences, but reduced robustness on out-of-distribution sample prediction problems \cite{robustness}. Because of these observations, we finally decided to train and test all our models using probabilistic labels. 
\subsection{Modeling}
Given the two prediction tasks at hand, we studied both no-reference image quality models and distortion classification models, with a goal of building multi-task models capable of both tasks.
\subsubsection{Image Quality Models}
\noindent\textbf{Architecture: }The model structure consists of a deep CNN backbone, followed by two-dimensional global average pooling, then two fully connected layers of size $512$ and $32$, respectively, and a single output neuron with sigmoid activation. The model was trained for $10$ epochs using Adam optimizer with MSE loss. The learning rate was set to $5\times 10^{-4}$ for the first 5 epoch, then with a decay rate of $0.1$ per epoch. We experimented with ResNet-50V2 \cite{resnet50v2}, Xception \cite{xception}, and ResNeXt-50 \cite{resnext} backbones pre-trained on ImageNet \cite{imageNet} and fine-tuned on LIVE-VizWiz. 

\noindent\textbf{Dataset Splits: }We used the same train-validation-test split as provided by the authors of VizWiz-QualityIssues \cite{vizwiz}. The training, validation, and testing set consists of $23.9$K ($60.3\%$), $7.7$K ($19.6\%$), and $8$K ($20.1\%$) images respectively. Similar split was applied to the patch dataset.

\noindent\textbf{Baselines and evaluation metrics: }The trained models were compared against several baselines, including shallow and deep learners. We included the popular image quality prediction models, BRISQUE \cite{brisque}, NIQE \cite{niqe}, and FRIQUEE \cite{friquee}, all of which we extract perceptually relevant statistical image features which are used to train an SVR. We also implemented two deep picture quality models -- CNNIQA \cite{cnnIqa} and NIMA \cite{nima} (with a VGG-16 \cite{vgg16} backbone and a single regressed quality score as output). Lastly, we also implemented the PaQ-2-PiQ baseline and PaQ-2-PiQ RoIPool \cite{paq2piq} models with backbones pre-trained on LIVE-FB, then fine-tuned on our dataset. Similar to all the standard work in the field of image quality assessment, we evaluated the performance of the models using the correlation metrics SRCC and LCC.

% \input{tbl/tbl_quality_models}

\noindent\textbf{Results: } 
The performances of the compared models have been summarized in Table \ref{tbl:quality_models}. Models trained with shallow learners on extracted features (BRISQUE \cite{brisque}, NIQE \cite{niqe}, and FRIQUEE \cite{friquee}) yielded lower prediction accuracy on our dataset as compared to the deep learners, which reflects the limited abilities of traditional features to capture the complex characteristics of distortions of natural images. CNNIQA \cite{cnnIqa}, which is a shallow CNN model, is able to outperform traditional algorithms, but falls short of the performances of deeper models. Among the remaining models, we observed that performance generally increased with depth, so deeper backbones (ResNet-50V2, ResNeXt-50, and Xception) outperformed NIMA \cite{nima} implemented with a VGG-16 backbone. Finally, the PaQ-2-PiQ RoIPool model achieved the best performance, demonstrating the efficacy of exploiting the relationship between local (patch) and global quality prediction. PaQ-2-PiQ only uses a ResNet-18 backbone. The performances of the deeper backbones were all similar (and close to the human performance -- SRCC $0.93$), suggesting that heavier models will not produce better performances. We considered whether the models were overfitting on VizWiz data, but the cross-dataset performance on ORBIT (Sec. \ref{sec:cross_data}) alleviated our concerns.

\subsubsection{Distortion Prediction Models}
\noindent\textbf{Architecture and Implementation: }
Because our models generates continuous probabilistic outputs, as described in Sec. \ref{sec:preprocess}, we treat distortion prediction as a regression problem. Similar to the quality model architecture, our proposed model consists of a deep CNN backbone, followed by global pooling, and two fully connected layers. Instead of producing a single output, our model has seven output neurons, each expressing a score a separate distortion class. As before, we experimented with three backbones - ResNet-50V2 \cite{resnet50v2}, Xception \cite{xception}, and ResNeXt-50 \cite{resnext}. 
% We also experimented with an RoIPool model similar to PaQ-2-PiQ \cite{paq2piq} but with distortion outputs (P2P-Dist). 
The hyperparameters were kept the same except that initial learning rate was modified to be $10^{-3}$. The same train-validation-test split was used. 

\noindent\textbf{Baselines and evaluation: }
The trained models were compared against other deep models. We include two models introduced in \cite{flickrdist}, where the authors used pre-trained Atrous VGG-16 \cite{atrvgg16} and ResNet-101 \cite{resNet} backbones with a single fully-connected head layer to predict synthetic distortions. We also the model proposed in \cite{vizwiz} composed of an Xception \cite{xception} backbone (pre-trained on ImageNet \cite{imageNet}), fine-tuning the head layers only. The distortion labels and outputs lie within [$0$,$1$], and we again used SRCC as the performance evaluation metric.

\noindent\textbf{Results: } As may be observed from Table \ref{tbl:dist_models}, the fine-tuned deep models outperformed the baselines. Atrous VGG-16 \cite{flickrdist} performed the worst among all, whereas the ResNet-50V2 \cite{resnet50v2} and ResNeXt-50 \cite{resnext} models consistently performed best on most distortion classes. All the fine-tuned models yielded similar performances across all classes. However, as discussed before, the distortion distribution in the dataset is quite skewed (Fig. \ref{fig:MOShists}), hence the prediction performances varied across classes. The low performance on the `bright' and `grainy' classes is consistent with the low agreement among the subjects on these distortions(Sec. \ref{sec:data_analysis}).
% \input{tbl/tbl_distortion_models}

\subsubsection{Multi-task Models}
\noindent\textbf{Architecture and Implementation: }
Combining both tasks -- quality and distortion type predictions -- into a single model bears two advantages -- fewer computations and faster inferencing, which is critical for supplying real-time  feedback to users (Sec. \ref{sec:feedback}), and shared distortion and quality features can lead to better predictions \cite{qualnet}. Starting with the PaQ-2-PiQ (P2P) RoIPool \cite{paq2piq} model as a base, we modified it by attaching a multi-task head to conduct quality and distortion prediction. The multi-task model, which we call P2P++, is able to produce quality and distortion predictions for each class, on both the entire image and each local patch simultaneously (Fig. \ref{fig:framework}). The multi-task head has a shared layer of size $512$, followed by two separate layers of size $32$, each dedicated to separate tasks. In addition to training P2P++ (which has a ResNet-18 \cite{resNet} backbone pre-trained on LIVE-FB \cite{paq2piq}), we also experimented with ResNet-50V2 \cite{resnet50v2} and Xception \cite{xception} backbone baselines. which were trained on images only. The hyperparameters for training were the same as for the distortion model setup, using the same train-validation-test split. 
% \input{fig/model_fig}

\noindent\textbf{Baselines and evaluation: } We compared the performance of our models against two multi-task deep models - IQACNN++ \cite{cnniqapp} and QualNet \cite{qualnet}. IQACNN++ consists of a shallow CNN backbone, whereas QualNet contains a VGG-16 \cite{vgg16} backbone and predicts global quality using fused distortion and quality features. As in the previous two sections, we again used the SRCC as the evaluation metric.   

\noindent\textbf{Results: } From Table \ref{tbl:multitask_models}, it may be observed that the shallow IQACNN++ \cite{cnniqapp} model yielded the worst results. QualNet \cite{qualnet} was able to outperform IQACNN++, but struggled on multiple distortion categories. The larger models equipped with ResNet-50V2 and Xception backbones performed very well, but the much lighter P2P++ model was able to achieve the best performance on almost all categories. Again, by inferencing on learned local-to-global quality and distortion features, better results are obtained at lower cost. As before, all of the models had more difficulty predicting the `bright' and `grainy' distortion types. Also comparing to Tables \ref{tbl:quality_models} and \ref{tbl:dist_models}, because of the shared features there is a slight improvement in quality prediction, although it is accompanied by a slight decrement of distortion prediction efficacy.
% \input{tbl/tbl_multitask_models}

\subsection{Other Experiments}
\noindent\textbf{Performance on patches:} 
Table \ref{tbl:patches} summarizes the performance of the multi-task models on patches. This is important, since giving feedback on local distortion occurences may further assist visually impaired users. P2P++ performs the best on both the random and salient patches, closely followed by ResNet-50V2. This validates the localization capabilities of the patch model. It is interesting to note that the performance on salient patches was slightly better than on random patches for most cases. This could be because salient patches often capture visibly obvious and annoying distortion information that might draw attention and is easier to predict (this is also suggested by the higher inter-subject consistencies observed in Sec. \ref{sec:data_analysis}). (Comments on distortion performance are included in Suppl.)
% \input{tbl/tbl_patch_results}

% \noindent\textbf{Random vs Salient patches:}
%Include if anything interesting to report

\noindent\textbf{Failure Cases:}
The image in Fig. \ref{fig:failure_eg} (a) was rated high (MOS = $76.2$) by the human subjects, but received a low predicted score (MOS = $50.2$) from P2P++. The reason for the low predicted score might be from the impact of the blurry regions on the hand and background, which is less noticeable than the high quality (salient) foreground. ``Bokeh" effects like this, which can be desirable, could be proactively modeled. On the other hand, the image in Fig. \ref{fig:failure_eg} (b) was rated as worse (MOS = $42.5$) by the human subjects than by P2P++ (MOS = $62.7$). A plausible reason for this discrepancy is the non-uniformity of the blur distortion across the image. While the sharp and distorted regions of the image are of roughly equal areas, the distortions were likely more salient to the human subjects, causing them to rate it more severely. However, the same regions wre likely predicted as less salient by P2P++. These results suggest that more work needs to be done, in this context, on understanding the interplay between saliency, distortion annoyance, and bokeh. Both of these examples show how non-uniform distortions of different natures can challenge even SOTA quality predictors like P2P++.

% \input{fig/failure_cases}



==> main_files/modeling_4.2.tex <==
\section{Applications of the proposed model} \label{sec:modelExt}
The models described on Sec. \ref{sec:modeling} can be extended to provide visualization and feedback to directly assist visually impaired users, which we describe next.
%The following sections describes some applications of our multi-task models directed towards our end goal of giving useful feedback to visually challenged users. 
\subsection{Predicting quality and distortion maps} \label{sec:qualityMaps}
The P2P++ model can be used to compute both spatial quality maps as well as distortion classification maps. Since it is trained on both global and local patch labels, it is flexible enough to compute the quality predictions and distortion type predictions any number and sizes of image patches. Inspired by the work in \cite{paq2piq}, we utilized these outputs to create perceptual quality and distortion classification maps that span the entire image dimension. To generate spatial quality maps, the image is divided into non-overlapping patches of size $N\times N$, on which predicted quality scores are obtained from the model output for every patch. Similarly, on each patch, a predicted distortion vector is obtained, with multiple values corresponding to each distortion type. Each distortion output can be used to generate a corresponding distortion-specific map. The patch size ($N$) is easily varied, allowing the generation of finer or coarser maps. 
% \deepti{The below is not clear to me. Is it important to be included?}
% In the current P2P++ model, there was an abundance of large images (and thus large patches cropped from them) in the new dataset, hence the accuracies of the prediction as the sizes of the patches are reduced. This is to be expected from statistical (small sample) considerations as well. We have observed that using patches where $N\sim 10\%$ of the linear image dimensions produces both accurate and reasonably localized predictions on VC-UGC images. 

For the purposes of visualization, we applied bi-linear interpolation to the generated maps to re-scale them to the input image dimensions.` 
To enhance visibility, the quality and distortion maps were transformed into `magma' and `cividis' colormaps respectively, which were then $\alpha$-blended ($\alpha = 0.8$) with the original image so that content-distortion alignments may be discerned.
Fig \ref{fig:space_quality_dist} shows the predicted quality and distortion maps (for the two most prominent predicted distortions) computed on a sample test image. The quality map accurately predicted the bottom-right part of the image to be of highest quality, while the distortion maps predicted bottom-left area to be blurry, and the top most region of the image to be underexposed. This example shows how perceived quality and distortion localization in an image affect each other.  
% \input{fig/fig_qmap_dist}

\subsection{Feedback to assist visually challenged} \label{sec:feedback}
\noindent\textbf{Guided Photography:}
Our overarching goal is to build a system that is able to provide feedback to visually challenged users so that they can take better pictures. This is of course a very challenging, multi-dimensional, and human-oriented problem, which will ultimately require extensive ergonomic and validation states with actual visually impaired users. We will describe our efforts in that direction further along. At this point, we have built a prototype early-stage, guided feedback system as a demonstration of how our work can be used to assist visually challenged users to take better photos. The currently implemented framework is illustrated in Fig. \ref{fig:guide_feedback}. The assistive model has two parts, a quality feedback loop and a distortion feedback loop. The high-level, immediate model outputs are an approximate English translation of the global picture quality prediction and expressions of the predicted distortion levels. Specifically, the user is provided an image rating from among `Bad' (0-20), `Poor' (20-40), `Fair' (40-60), `Good' (60-80), and 'Excellent' (80-100). If the user is satisfied with the quality, he/she can choose to save it, or ask for distortion feedback otherwise. In our current prototype which is implemented on a workstation (but see below for parallel work), the feedback is given by output text; naturally, transcribed audio expression will be used in practice. If the quality is substandard, then further feedback is required to make the application useful. If feedback on the distortion is requested, the user is informed of the three major distortions determined to be present in the image, along with the severity of each: High ($> 0.50$), Moderate ($0.20 - 0.50$), and Low ($< 0.20$). 

Based on the nature and severities of the distortions detected, our system also suggests simple ways to mitigate the distortions: `blur' - `Move the phone away from the object,' `shaky' - `Keep the phone steady,' and so on. These comprise the base feedback of our prototype system. As the user becomes more adept at the P2P++ system, they will be able to request and take advantage of additional, more detailed feedback on the picture distortions. To facilitate this, P2P++ also generates $3\times 3$ distortion maps for the three most dominant impairments, and informs the user of their relative location in the image (top-left, bottom-right, center, etc.), as also depicted in Fig. \ref{fig:guide_feedback}.
% \input{fig/guide_feedback_framework}

\noindent\textbf{Automated Photography: }
Although guided photography promises to be a transformative technology, we acknowledge that much work remains in terms of developing an ideal feedback language and interface, which in term will require working with visually challenged subjects to test and advance the system. In the interim, there are more immediate ways to assist visually challenged users to take better pictures via a much simpler, albeit less comprehensive application, which can automatically help them take a better quality photo. This can be accomplished by capturing a short video clip of the scene the subject is trying to photograph, that includes and is approximately centered at the moment the `shutter button' is depressed. By using a broad sampling of a single frame per second, a fairly wide range of qualities may be presented. Given the sampled frames, P2P++ then computes the global quality of each to determine the frame having the highest perceptual quality. The user is provided a feedback on this quality (`Poor' to `Excellent') and given the option to save the image. A simple demonstration on an ORBIT \cite{orbit} video is shown in Fig. \ref{fig:auto_feedback}. 
% \input{fig/auto_feedback}

\noindent\textbf{Performance on LIVE-ORBIT} \label{sec:cross_data}
To study the generalizability of our model, and the representation capabilities of our dataset, we also sought to test P2P++ on other, independent VC-UGC data than our new dataset. Since we could not find any other such datasets, we evaluated and compared the multi-task models on a special-purpose excerpt we created from the ORBIT dataset (Sec. \ref{dataset}), consisting of frame images sampled from the ORBIT \cite{orbit} videos. As may be observed from Table \ref{tbl:orbit_results}, P2P++ performs very well, and generally better than the much heavier ResNet-50V2 and Xception models. All the models that we have created outperform other multi-task models when trained on our proposed new database and tested on the excerpted ORBIT dataset. Attaining such high performance on most distortion classes on ORBIT validates the generalizability of P2P++ to other VC-UGC media. The lower performance on the `bright' and `grainy' categories (of all models) might be attributed to a mismatch of distortion distributions between the two populations. Finally, Fig. \ref{fig:auto_feedback} illustrates the actual performance and outputs produced by P2P++ when compared to the ground truth quality scores obtained on an ORBIT video.

% \input{tbl/tbl_orbit_results}


==> modeling_files/modeling_4.1.tex <==
\section{Modeling and Experiments}\label{sec:modeling}
Our goal is to create an application which can accurately predict and accordingly provide feedback on the perceptual quality and distortions present in a picture. Towards this end, we designed efficient model architectures able to predict quality and distortions, while accounting for local-to-global percepts. Our model is able to analyze quality and distortion types both separately and together in a  multi-task framework. 
\subsection{Data pre-processing}\label{sec:preprocess}
Unlike the quality scores, which could be used in their raw form, the distortion labels had to be transformed into suitable output labels for training. Since distortion type prediction is a classification task, binarizing the labels was our first choice. We considered multiple options to decide a threshold on the per-distortion proportions of ratings. The authors of \cite{vizwiz} considered $40\%$ ($2$ out of $5$) agreement to affirm the presence of a distortion. Since there were no perceptual principles to guide us, we experimented with three thresholds values: $0.3$, $0.4$, and $0.5$ and assumed the top three distortions (highest proportions of the total number of labels) to be present. An inter-subject consistency analysis on the binarized labels found that the SRCC values dropped by $17\%$--$34\%$ as compared to those obtained on the probabilistic values in Sec. \ref{sec:data_analysis}. Similarly, we noticed a drop of $27\%$--$44\%$ of correlation between assigned patch vs image distortion classes, as compared to the probabilistic approach. Among all the binarization strategies, the `max-three' approach led to the worst correlation values. Moreover, as the thresholds were increased, the distortion distributions became more skewed, leading to worse predictions. These results made sense in view of research on model robustness, which has shown that, for classification tasks, hard labels tend to lead to higher confidences, but reduced robustness on out-of-distribution sample prediction problems \cite{robustness}. Because of these observations, we finally decided to train and test all our models using probabilistic labels. 
\subsection{Modeling}
Given the two prediction tasks at hand, we studied both no-reference image quality models and distortion classification models, with a goal of building multi-task models capable of both tasks.
\subsubsection{Image Quality Models}
\noindent\textbf{Architecture: }The model structure consists of a deep CNN backbone, followed by two-dimensional global average pooling, then two fully connected layers of size $512$ and $32$, respectively, and a single output neuron with sigmoid activation. The model was trained for $10$ epochs using Adam optimizer with MSE loss. The learning rate was set to $5\times 10^{-4}$ for the first 5 epoch, then with a decay rate of $0.1$ per epoch. We experimented with ResNet-50V2 \cite{resnet50v2}, Xception \cite{xception}, and ResNeXt-50 \cite{resnext} backbones pre-trained on ImageNet \cite{imageNet} and fine-tuned on LIVE-VizWiz. 

\noindent\textbf{Dataset Splits: }We used the same train-validation-test split as provided by the authors of VizWiz-QualityIssues \cite{vizwiz}. The training, validation, and testing set consists of $23.9$K ($60.3\%$), $7.7$K ($19.6\%$), and $8$K ($20.1\%$) images respectively. Similar split was applied to the patch dataset.

\noindent\textbf{Baselines and evaluation metrics: }The trained models were compared against several baselines, including shallow and deep learners. We included the popular image quality prediction models, BRISQUE \cite{brisque}, NIQE \cite{niqe}, and FRIQUEE \cite{friquee}, all of which we extract perceptually relevant statistical image features which are used to train an SVR. We also implemented two deep picture quality models -- CNNIQA \cite{cnnIqa} and NIMA \cite{nima} (with a VGG-16 \cite{vgg16} backbone and a single regressed quality score as output). Lastly, we also implemented the PaQ-2-PiQ baseline and PaQ-2-PiQ RoIPool \cite{paq2piq} models with backbones pre-trained on LIVE-FB, then fine-tuned on our dataset. Similar to all the standard work in the field of image quality assessment, we evaluated the performance of the models using the correlation metrics SRCC and LCC.

\input{tbl/tbl_quality_models}

\noindent\textbf{Results: } 
The performances of the compared models have been summarized in Table \ref{tbl:quality_models}. Models trained with shallow learners on extracted features (BRISQUE \cite{brisque}, NIQE \cite{niqe}, and FRIQUEE \cite{friquee}) yielded lower prediction accuracy on our dataset as compared to the deep learners, which reflects the limited abilities of traditional features to capture the complex characteristics of distortions of natural images. CNNIQA \cite{cnnIqa}, which is a shallow CNN model, is able to outperform traditional algorithms, but falls short of the performances of deeper models. Among the remaining models, we observed that performance generally increased with depth, so deeper backbones (ResNet-50V2, ResNeXt-50, and Xception) outperformed NIMA \cite{nima} implemented with a VGG-16 backbone. Finally, the PaQ-2-PiQ RoIPool model achieved the best performance, demonstrating the efficacy of exploiting the relationship between local (patch) and global quality prediction. PaQ-2-PiQ only uses a ResNet-18 backbone. The performances of the deeper backbones were all similar (and close to the human performance -- SRCC $0.93$), suggesting that heavier models will not produce better performances. We considered whether the models were overfitting on VizWiz data, but the cross-dataset performance on ORBIT (Sec. \ref{sec:cross_data}) alleviated our concerns.

\subsubsection{Distortion Prediction Models}
\noindent\textbf{Architecture and Implementation: }
Because our models generates continuous probabilistic outputs, as described in Sec. \ref{sec:preprocess}, we treat distortion prediction as a regression problem. Similar to the quality model architecture, our proposed model consists of a deep CNN backbone, followed by global pooling, and two fully connected layers. Instead of producing a single output, our model has seven output neurons, each expressing a score a separate distortion class. As before, we experimented with three backbones - ResNet-50V2 \cite{resnet50v2}, Xception \cite{xception}, and ResNeXt-50 \cite{resnext}. 
% We also experimented with an RoIPool model similar to PaQ-2-PiQ \cite{paq2piq} but with distortion outputs (P2P-Dist). 
The hyperparameters were kept the same except that initial learning rate was modified to be $10^{-3}$. The same train-validation-test split was used. 

\noindent\textbf{Baselines and evaluation: }
The trained models were compared against other deep models. We include two models introduced in \cite{flickrdist}, where the authors used pre-trained Atrous VGG-16 \cite{atrvgg16} and ResNet-101 \cite{resNet} backbones with a single fully-connected head layer to predict synthetic distortions. We also the model proposed in \cite{vizwiz} composed of an Xception \cite{xception} backbone (pre-trained on ImageNet \cite{imageNet}), fine-tuning the head layers only. The distortion labels and outputs lie within [$0$,$1$], and we again used SRCC as the performance evaluation metric.

\noindent\textbf{Results: } As may be observed from Table \ref{tbl:dist_models}, the fine-tuned deep models outperformed the baselines. Atrous VGG-16 \cite{flickrdist} performed the worst among all, whereas the ResNet-50V2 \cite{resnet50v2} and ResNeXt-50 \cite{resnext} models consistently performed best on most distortion classes. All the fine-tuned models yielded similar performances across all classes. However, as discussed before, the distortion distribution in the dataset is quite skewed (Fig. \ref{fig:MOShists}), hence the prediction performances varied across classes. The low performance on the `bright' and `grainy' classes is consistent with the low agreement among the subjects on these distortions(Sec. \ref{sec:data_analysis}).
\input{tbl/tbl_distortion_models}

\subsubsection{Multi-task Models}
\noindent\textbf{Architecture and Implementation: }
Combining both tasks -- quality and distortion type predictions -- into a single model bears two advantages -- fewer computations and faster inferencing, which is critical for supplying real-time  feedback to users (Sec. \ref{sec:feedback}), and shared distortion and quality features can lead to better predictions \cite{qualnet}. Starting with the PaQ-2-PiQ (P2P) RoIPool \cite{paq2piq} model as a base, we modified it by attaching a multi-task head to conduct quality and distortion prediction. The multi-task model, which we call P2P++, is able to produce quality and distortion predictions for each class, on both the entire image and each local patch simultaneously (Fig. \ref{fig:framework}). The multi-task head has a shared layer of size $512$, followed by two separate layers of size $32$, each dedicated to separate tasks. In addition to training P2P++ (which has a ResNet-18 \cite{resNet} backbone pre-trained on LIVE-FB \cite{paq2piq}), we also experimented with ResNet-50V2 \cite{resnet50v2} and Xception \cite{xception} backbone baselines. which were trained on images only. The hyperparameters for training were the same as for the distortion model setup, using the same train-validation-test split. 
\input{fig/model_fig}

\noindent\textbf{Baselines and evaluation: } We compared the performance of our models against two multi-task deep models - IQACNN++ \cite{cnniqapp} and QualNet \cite{qualnet}. IQACNN++ consists of a shallow CNN backbone, whereas QualNet contains a VGG-16 \cite{vgg16} backbone and predicts global quality using fused distortion and quality features. As in the previous two sections, we again used the SRCC as the evaluation metric.   

\noindent\textbf{Results: } From Table \ref{tbl:multitask_models}, it may be observed that the shallow IQACNN++ \cite{cnniqapp} model yielded the worst results. QualNet \cite{qualnet} was able to outperform IQACNN++, but struggled on multiple distortion categories. The larger models equipped with ResNet-50V2 and Xception backbones performed very well, but the much lighter P2P++ model was able to achieve the best performance on almost all categories. Again, by inferencing on learned local-to-global quality and distortion features, better results are obtained at lower cost. As before, all of the models had more difficulty predicting the `bright' and `grainy' distortion types. Also comparing to Tables \ref{tbl:quality_models} and \ref{tbl:dist_models}, because of the shared features there is a slight improvement in quality prediction, although it is accompanied by a slight decrement of distortion prediction efficacy.
\input{tbl/tbl_multitask_models}

\subsection{Other Experiments}
\noindent\textbf{Performance on patches:} 
Table \ref{tbl:patches} summarizes the performance of the multi-task models on patches. This is important, since giving feedback on local distortion occurences may further assist visually impaired users. P2P++ performs the best on both the random and salient patches, closely followed by ResNet-50V2. This validates the localization capabilities of the patch model. It is interesting to note that the performance on salient patches was slightly better than on random patches for most cases. This could be because salient patches often capture visibly obvious and annoying distortion information that might draw attention and is easier to predict (this is also suggested by the higher inter-subject consistencies observed in Sec. \ref{sec:data_analysis}). (Comments on distortion performance are included in Suppl.)
\input{tbl/tbl_patch_results}

% \noindent\textbf{Random vs Salient patches:}
%Include if anything interesting to report

\noindent\textbf{Failure Cases:}
The image in Fig. \ref{fig:failure_eg} (a) was rated high (MOS = $76.2$) by the human subjects, but received a low predicted score (MOS = $50.2$) from P2P++. The reason for the low predicted score might be from the impact of the blurry regions on the hand and background, which is less noticeable than the high quality (salient) foreground. ``Bokeh" effects like this, which can be desirable, could be proactively modeled. On the other hand, the image in Fig. \ref{fig:failure_eg} (b) was rated as worse (MOS = $42.5$) by the human subjects than by P2P++ (MOS = $62.7$). A plausible reason for this discrepancy is the non-uniformity of the blur distortion across the image. While the sharp and distorted regions of the image are of roughly equal areas, the distortions were likely more salient to the human subjects, causing them to rate it more severely. However, the same regions wre likely predicted as less salient by P2P++. These results suggest that more work needs to be done, in this context, on understanding the interplay between saliency, distortion annoyance, and bokeh. Both of these examples show how non-uniform distortions of different natures can challenge even SOTA quality predictors like P2P++.

\input{fig/failure_cases}



==> modeling_files/modeling_4.2.tex <==
\section{Applications of the proposed model} \label{sec:modelExt}
The models described on Sec. \ref{sec:modeling} can be extended to provide visualization and feedback to directly assist visually impaired users, which we describe next.
%The following sections describes some applications of our multi-task models directed towards our end goal of giving useful feedback to visually challenged users. 
\subsection{Predicting quality and distortion maps} \label{sec:qualityMaps}
The P2P++ model can be used to compute both spatial quality maps as well as distortion classification maps. Since it is trained on both global and local patch labels, it is flexible enough to compute the quality predictions and distortion type predictions any number and sizes of image patches. Inspired by the work in \cite{paq2piq}, we utilized these outputs to create perceptual quality and distortion classification maps that span the entire image dimension. To generate spatial quality maps, the image is divided into non-overlapping patches of size $N\times N$, on which predicted quality scores are obtained from the model output for every patch. Similarly, on each patch, a predicted distortion vector is obtained, with multiple values corresponding to each distortion type. Each distortion output can be used to generate a corresponding distortion-specific map. The patch size ($N$) is easily varied, allowing the generation of finer or coarser maps. 
\deepti{The below is not clear to me. Is it important to be included?}
In the current P2P++ model, there was an abundance of large images (and thus large patches cropped from them) in the new dataset, hence the accuracies of the prediction as the sizes of the patches are reduced. This is to be expected from statistical (small sample) considerations as well. We have observed that using patches where $N\sim 10\%$ of the linear image dimensions produces both accurate and reasonably localized predictions on VC-UGC images. 

\textcolor{green}{For the purposes of visualization, we applied bi-linear interpolation to the generated maps to re-scale them to the input image dimensions. 
To enhance visibility, the quality and distortion maps were transformed into `magma' and `cividis' colormaps respectively, which were then $\alpha$-blended ($\alpha = 0.8$) with the original image so that content-distortion alignments may be discerned. }
Fig \ref{fig:space_quality_dist} shows the predicted quality and distortion maps (for the two most prominent predicted distortions) computed on a sample test image. The quality map accurately predicted the bottom-right part of the image to be of highest quality, while the distortion maps predicted bottom-left area to be blurry, and the top most region of the image to be underexposed. This example shows how perceived quality and distortion localization in an image affect each other.  
\input{fig/fig_qmap_dist}

\subsection{Feedback to assist visually challenged} \label{sec:feedback}
\noindent\textbf{Guided Photography:}
Our overarching goal is to build a system that is able to provide feedback to visually challenged users so that they can take better pictures. This is of course a very challenging, multi-dimensional, and human-oriented problem, which will ultimately require extensive ergonomic and validation states with actual visually impaired users. We will describe our efforts in that direction further along. At this point, we have built a prototype early-stage, guided feedback system as a demonstration of how our work can be used to assist visually challenged users to take better photos. The currently implemented framework is illustrated in Fig. \ref{fig:guide_feedback}. The assistive model has two parts, a quality feedback loop and a distortion feedback loop. The high-level, immediate model outputs are an approximate English translation of the global picture quality prediction and expressions of the predicted distortion levels. Specifically, the user is provided an image rating from among `Bad' (0-20), `Poor' (20-40), `Fair' (40-60), `Good' (60-80), and 'Excellent' (80-100). If the user is satisfied with the quality, he/she can choose to save it, or ask for distortion feedback otherwise. In our current prototype which is implemented on a workstation (but see below for parallel work), the feedback is given by output text; naturally, transcribed audio expression will be used in practice. If the quality is substandard, then further feedback is required to make the application useful. If feedback on the distortion is requested, the user is informed of the three major distortions determined to be present in the image, along with the severity of each: High ($> 0.50$), Moderate ($0.20 - 0.50$), and Low ($< 0.20$). 

Based on the nature and severities of the distortions detected, our system also suggests simple ways to mitigate the distortions: `blur' - `Move the phone away from the object,' `shaky' - `Keep the phone steady,' and so on. These comprise the base feedback of our prototype system. As the user becomes more adept at the P2P++ system, they will be able to request and take advantage of additional, more detailed feedback on the picture distortions. To facilitate this, P2P++ also generates $3\times 3$ distortion maps for the three most dominant impairments, and informs the user of their relative location in the image (top-left, bottom-right, center, etc.), as also depicted in Fig. \ref{fig:guide_feedback}.
\input{fig/guide_feedback_framework}

\noindent\textbf{Automated Photography: }
Although guided photography promises to be a transformative technology, we acknowledge that much work remains in terms of developing an ideal feedback language and interface, which in term will require working with visually challenged subjects to test and advance the system. In the interim, there are more immediate ways to assist visually challenged users to take better pictures via a much simpler, albeit less comprehensive application, which can automatically help them take a better quality photo. This can be accomplished by capturing a short video clip of the scene the subject is trying to photograph, that includes and is approximately centered at the moment the `shutter button' is depressed. By using a broad sampling of a single frame per second, a fairly wide range of qualities may be presented. Given the sampled frames, P2P++ then computes the global quality of each to determine the frame having the highest perceptual quality. The user is provided a feedback on this quality (`Poor' to `Excellent') and given the option to save the image. A simple demonstration on an ORBIT \cite{orbit} video is shown in Fig. \ref{fig:auto_feedback}. 
\input{fig/auto_feedback}

\noindent\textbf{Performance on LIVE-ORBIT} \label{sec:cross_data}
To study the generalizability of our model, and the representation capabilities of our dataset, we also sought to test P2P++ on other, independent VC-UGC data than our new dataset. Since we could not find any other such datasets, we evaluated and compared the multi-task models on a special-purpose excerpt we created from the ORBIT dataset (Sec. \ref{dataset}), consisting of frame images sampled from the ORBIT \cite{orbit} videos. As may be observed from Table \ref{tbl:orbit_results}, P2P++ performs very well, and generally better than the much heavier ResNet-50V2 and Xception models. All the models that we have created outperform other multi-task models when trained on our proposed new database and tested on the excerpted ORBIT dataset. Attaining such high performance on most distortion classes on ORBIT validates the generalizability of P2P++ to other VC-UGC media. The lower performance on the `bright' and `grainy' categories (of all models) might be attributed to a mismatch of distortion distributions between the two populations. Finally, Fig. \ref{fig:auto_feedback} illustrates the actual performance and outputs produced by P2P++ when compared to the ground truth quality scores obtained on an ORBIT video.

\input{tbl/tbl_orbit_results}

